MolReasoner: Toward Effective and Interpretable Reasoning for Molecular LLMs

Large Language Models (LLMs) have shown impressive performance across various domains, but their ability to perform molecular reasoning remains underexplored. Existing methods mostly rely on general-purpose prompting, which lacks domain-specific molecular semantics, or fine-tuning, which faces challenges in interpretability and reasoning depth, often leading to structural and textual hallucinations. To address these issues, we introduce MolReasoner, a two-stage framework that transitions LLMs from memorization to high-fidelity chemical reasoning. In the Mol-SFT stage, knowledge-enhanced Chain-of-Thought (CoT) data provides a strong foundation, while the Mol-RL stage refines reasoning using a novel, task-adaptive reward system to mitigate hallucinations. Extensive evaluations demonstrate that MolReasoner significantly outperforms a wide range of strong baselines in both molecule generation and captioning tasks. Further analyses highlight the framework's synergistic design and its ability to produce more interpretable outputs. Our work presents a principled and effective new approach for advancing high-fidelity molecular reasoning.

==> chapters/3_prelim.tex <==
\section{Preliminary}
A comprehensive review of related work on molecular language models and large reasoning models is provided in the appendix. 
In this section, we briefly describe the molecular understanding task -- \textit{molecule-text translation}—and outline the reinforcement learning approach, \textit{Group Relative Policy Optimization (GRPO)}, employed in MolReasoner.

\subsection{Molecule-Text Translation}
Advancing the use of LLMs in molecular science requires moving beyond structural representations toward explicit structure-level reasoning grounded in natural language.
Such reasoning abilities are essential for interpreting molecular semantics, inferring molecular functions, and generating chemically plausible structures from textual inputs.
To systematically evaluate these capabilities,  researchers~\cite{molt5} introduced the \textit{molecule-text translation} task, designed to assess a model’s proficiency in aligning and reasoning between molecular representations and natural language descriptions. 
This task comprises two complementary sub-tasks:
\begin{itemize}
\item \textbf{Molecule Captioning}: Given a molecular descriptor (\eg SMILES~\cite{smiles}, SELFIES~\cite{selfies}, or IUPAC name~\cite{iupac}), the objective is to generate a coherent natural-language description capturing structural characteristics, functional roles, and potential applications of the molecule. 
This evaluates the model's ability to interpret molecular structures and abstract their semantics into text.
\item \textbf{Text-based de novo Molecule Generation}: Conversely, this task requires the model to generate valid molecular descriptors from natural language descriptions, testing its capacity to map textual semantics to relevant chemical motifs, and produce syntactically and chemically valid molecular structures.
\end{itemize}
Previous studies~\cite{galactica,molt5} uses SMILES for molecule representation, its grammar and token order sensitivity often result in invalid or chemically implausible outputs. 
primarily employed SMILES for molecular representation. However, the grammar and token-order sensitivity inherent in SMILES frequently lead to invalid or chemically implausible outputs. To overcome this limitation, we adopt SELFIES representations, following the Mol-Instructions framework~\cite{mol-instruction}. 
SELFIES ensures chemical validity by construction, eliminating common structural errors such as mismatched parentheses, invalid atomic symbols, and illogical branching patterns.

\subsection{Group Relative Policy Optimization}
The core innovation of Group Relative Policy Optimization (GRPO)~\cite{deepseekmath} lies in its group-based redefinition of the advantage function.
In contrast to PPO, GRPO removes the value function and estimates advantages relative to a sampled response group.
Specifically, given a question-answer pair $(q,a)$, the old policy $\pi_{\theta_\text{old}}$ samples a group of $G$ responses $\{ o_i\}_{i=1}^G$. 
The advantage for the $i$-th response is computed by normalizing the corresponding group-level rewards $\{ R_i \}_{i=1}^G$:
\begin{equation}
\hat{A}_{i,t} = \frac{r_i - \text{mean}(\{R_i\}_{i=1}^G)}{\text{std}(\{R_i\}_{i=1}^G)}.
\end{equation}

Additionally, GRPO employs a clipped objective combined with a KL-divergence penalty term, defined as:
\begin{equation}
\begin{aligned}
\mathcal{J}_\text{GRPO}(\theta) &= 
\mathbb{E}_{(q,a)\sim \mathcal{D}, \{o_i\}_{i=1}^G \sim \pi_{\theta_\text{old}}(\cdot\mid q)} \Bigg[
\frac{1}{G}\sum_{i=1}^{G} \frac{1}{|o_i|} \sum_{t=1}^{|o_i|} \Bigg( \\
&\quad \min \Big( r_{i,t}(\theta) \hat{A}_{i,t},\ 
\text{clip} \left( r_{i,t}(\theta), 1 - \varepsilon, 1 + \varepsilon \right) \hat{A}_{i,t} \Big) \\
&\quad - \beta D_{\text{KL}}(\pi_{\theta} \parallel \pi_{\text{ref}}) 
\Bigg) \Bigg]
\end{aligned}
\label{eq:grpoloss}
\end{equation}
where the importance ratio $r_{i,t}(\theta)$ is given by:
\begin{equation}
    r_{i,t}(\theta)=\frac{\pi_{\theta}(o_{i,t} \mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t} \mid q,o_{i,<t})}.
\end{equation}



==> chapters/8_checklist.tex <==
\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

\ifreproStandalone

\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}

\frenchspacing


\fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}

\section*{Reproducibility Checklist}

% The questions start here

\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
yes

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
yes

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
yes

\end{itemize}
\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
no

	\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
        \begin{itemize}
	
	\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
	NA

	\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
	NA

	\question{Proofs of all novel claims are included}{(yes/partial/no)}
	NA

	\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
	NA

	\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
	NA

	\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
	NA

	\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
	NA
	
	\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
	yes

	\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
	NA

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
	yes

	\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
	yes
        
	\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
	yes

	\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
	yes

	\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
	yes

	\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
	yes

	\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
	no

	\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
	no

	\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
	no

	\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments}{(yes/partial/no/NA)}
	yes


\end{itemize}
\end{itemize}
\ifreproStandalone

